Optimal Strategies for Communication and Remote Estimation with an Energy Harvesting Sensor

We consider a remote estimation problem with an energy harvesting sensor and a remote estimator. The sensor observes the state of a discrete-time source which may be a finite state Markov chain or a multi-dimensional linear Gaussian system. It harvests energy from its environment (say, for example, through a solar cell) and uses this energy for the purpose of communicating with the estimator. Due to the randomness of energy available for communication, the sensor may not be able to communicate all the time. The sensor may also want to save its energy for future communications. The estimator relies on messages communicated by the sensor to produce real-time estimates of the source state. We consider the problem of finding a communication scheduling strategy for the sensor and an estimation strategy for the estimator that jointly minimize an expected sum of communication and distortion costs over a finite time horizon. Our goal of joint optimization leads to a decentralized decision-making problem. By viewing the problem from the estimator's perspective, we obtain a dynamic programming characterization for the decentralized decision-making problem that involves optimization over functions. Under some symmetry assumptions on the source statistics and the distortion metric, we show that an optimal communication strategy is described by easily computable thresholds and that the optimal estimate is a simple function of the most recently received sensor observation.

==> gaussian_v2.tex <==
\section{Multi-dimensional Gaussian Source} \label{sec:multi_d}

In this section, we consider Problem \ref{prob:main} with a  multi-dimensional Gaussian source. The state of the source evolves according to the equation
\begin{equation}
\VEC X_{t+1} = \lambda\VEC A\VEC X_t + \VEC Z_t,
\end{equation}
where   $\VEC{X}_t =(X^1_t,X^2_t,\ldots,X^n_t)$, $\VEC{Z}_t =(Z^1_t,Z^2_t,\ldots,Z^n_t)$ are random vectors taking values in $\mathbb{R}^n$, $\lambda > 0$ is a real number and $\VEC A$ is an orthogonal matrix (that is, transpose of $\VEC A$ is the inverse of $\VEC A$ and, more importantly for our analysis, $\VEC A$ preserves norms). The initial state $\VEC X_1$ has a zero-mean Gaussian distribution with variance $s_1 \VEC I$ and $\VEC Z_1, \VEC Z_2,...,\VEC Z_{T-1}$ are i.i.d. random vectors with a zero-mean Gaussian distribution and variance $s_2 \VEC I$. The energy dynamics for the sensor as the same as in Problem \ref{prob:main}. 

 At the beginning of the time period $t$, the sensor makes a decision about whether to transmit its current observation vector and its current energy level to the estimator or not. %We denote by $U_t \in \{0,1\}$ the sensor's decision at time $t$, where $U_t=0$ means no transmission and $U_t=1$ means a decision to transmit. 
The estimator receives a message $Y_t$ from the sensor where
\begin{align}
Y_t = \left \{ \begin{array}{ll}
               (\VEC{X}_t,E_t) & \mbox{if $U_t =1$} \\
               \epsilon & \mbox{ if $U_t=0$ },
               \end{array}
               \right.
\end{align} 
where $\epsilon$ denotes that no message was transmitted.
The estimator produces an estimate $\VEC{\hat{X}}_t = (\hat{X}^1_t,\ldots, \hat{X}^n_t)$ at time $t$ depending on the sequence of messages it received so far. The system operates for a finite time horizon $T$.

The sensor and estimator make their decisions according to deterministic strategies $\VEC f$ and $\VEC g$, that is,
\[ U_t = f_t(X_t,E_t,Y_{1:t-1}) \]
and \[ \hat{\VEC{X}}_t = g_t(Y_{1:t})\]
 
We have the following optimization problem.

\begin{problem}
  \label{prob:multi_d}
  For the model described above, given the statistics of the Markov source and the initial energy level $E_1$, the statistics of amounts of energy harvested at each time, the sensor's energy storage limit $B$ and the time horizon $T$,  find  decision strategies $\VEC f, \VEC g$ for the sensor and the estimator that minimize the following expected cost:
  \begin{equation}\label{eq:mcost}
  J(\VEC f, \VEC g) = \mathds{E} \{\sum_{t=1}^T c U_t + \norm{\VEC{X}_t-\VEC{\hat {X}}_t}^2 \},
  \end{equation}
 where $c \geq 0$ is a communication cost and $\norm{\cdot}$ is the Euclidean norm. 
\end{problem}
\begin{remark}
Note that we have assumed here that sensor is using a deterministic strategy that only uses the current source and energy state and the past transmissions to make the decision at time $t$. Using arguments analogous to those used in proving Lemma \ref{lemma:str}, it can be shown that this restriction is without loss of optimality.
\end{remark}
%Consider a strategy $\VEC f$ of the sensor. We call a realization $y_{1:t}$ of the transmissions from time $1$ to $t$ as a \emph{possible realization} if there exists a sequence of source states and energy levels $x_{1:t},e_{1:t}$ such that $y_s=f_s(x_s,e_s,y_{1:s-1})$, $1 \leq s \leq t$. (For example, if the sensor strategy is to always transmit at time $t$, a realization with $y_t=\epsilon$ is not a possible realization.) Let $s \leq (t-1)$ be the most recent time such that $y_s \neq \epsilon$. Let $y_s=(x_s,e_s)$. We can then define at time $t$, a pre-transmission belief on $\VEC X_t,E_t$ as
%\[ \mathds{P}(\VEC X_t \in A, E_t =e) = \mathds{P}((x_s+\VEC Z_s+\VEC Z_{s+1}+\ldots,+\VEC Z_{t-1}) \in A, (e_s-1+N_s+\ldots+N_{t-1}) = e|)
%We make the following technical assumption.
%\begin{assumption}
%We consider sensor strategies such that for any time $t$,
%\begin{enumerate}
%\item The conditional probability measure on $\VEC X_t$ given the past transmissions, $y_{1:t-1}$, is absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^n$.
%\item The conditional probability measure on $\VEC X_t$ given the transmissions till time $t$, $y_{1:t}$, is either a delta distribution at some point $\VEC x$ or it is absolutely continuous with respect to the Lebesgue measure on $\mathbb{R}^n$.
%\end{enumerate} 
%\end{assumption}


\begin{definition}
 A function $\nu: \mathbb{R}^n \mapsto \mathds{R}$  is said to be \emph{ symmetric and unimodal} about a point $\VEC{a} \in \mathbb{R}^n$, if $\norm{\VEC{x-a}} \leq \norm{\VEC{y-a}}$ implies that $\nu(\VEC{x}) \geq \nu(\VEC{y})$. Further, we use the convention that a Dirac-delta function at $\VEC a$ is also symmetric unimodal about $\VEC a$.  
\end{definition}
For a Borel set $A$ in $\mathbb{R}^n$, we denote by $\mathcal{L}(A)$ the Lesbesgue measure of $A$. 
\begin{definition}
For a Borel set $A$ in $\mathbb{R}^n$, we denote by $A^{\sigma}$ the symmetric rearrangement of $A$. That is, $A^{\sigma}$ is an open ball centered at $\VEC 0$ whose volume is $\mathcal{L}(A)$. Given an integrable, non-negative function $h: \mathbb{R}^n \mapsto \mathbb{R}$, we denote by $h^{\sigma}$ its symmetric non-decreasing rearrangement. That is, 
\[ h^{\sigma}(x) = \int_0^{\infty}\mathds{1}_{\{\VEC a \in \mathbb{R}^n|h(\VEC a) > t\}^{\sigma}}(x)dt \]
\end{definition}
\begin{definition}
 Given two integrable, non-negative functions $h_1$ and $h_2$ from $\mathbb{R}^n$ to $\mathbb{R}$, we say that $h_1$ majorizes $h_2$, denoted by, $h_2 \prec h_1$, if the following holds:
\begin{align*}
\int_{\norm{\VEC x}\leq t}h_2^{\sigma}(\VEC x)d\VEC x \leq \int_{\norm{\VEC x}\leq t}h_1^{\sigma}(\VEC x)d\VEC x \mbox{~~~~$\forall t>0$}
\end{align*}
and
\begin{align*}
\int_{\mathbb{R}^n}h_2^{\sigma}(\VEC x)d\VEC x = \int_{\mathbb{R}^n}h_1^{\sigma}(\VEC x)d\VEC x \mbox{~~~~$\forall t>0$}
\end{align*}
Further, if $\int_{\mathbb{R}^n}h_2^{\sigma}(\VEC x)d\VEC x = c$, we say that $h^2 \prec c\delta(\VEC a)$, where $\delta(\VEC a)$ is the Dirac delta function at $\VEC a$ for any $\VEC a \in \mathbb{R}^n$. Further, for any $\VEC a, \VEC b$ and for any positive real number $c$, we say that $c\delta(\VEC b) \prec c\delta(\VEC a)$. 
\end{definition}


Following the arguments of Sections \ref{sec:prelim} and \ref{sec:results}, we can view the problem from the estimator's perspective who at each time $t$ selects a prescription for the sensor before the transmission and then an estimate on the source after the transmission. Because we have deterministic policies, the prescriptions are binary-valued functions. We can define at each time $t$,  the estimator's pre-transmission (post-transmission) beliefs as conditional probability measures on  $\mathbb{R}^n \times \mathcal{E}$ given the transmissions $Y_{1:t-1}$ ($Y_{1:t}$). Note that at time $t=1$, the pre-transmission belief on the source is described by a Gaussian density. Consider any (measurable) strategy such that the probability of $U_1=0$ is non-zero. Then, the post-transmission belief on source given $U_1=0$ is described by a density. Further, the pre-transmission belief on source at time $t=2$ given $U_1=0$ will also be associated with a density. In case a transmission happens, the post transmission belief on source is a Dirac-delta function and the pre-transmission belief on source at time $t=2$ will be associated with a density.  Thus, the pre-transmission belief on source is always described by a density function  and the post-transmission belief on the source is always either a delta function or it is described by a density. Treating the delta function as a density as well, we will use the terms pre-transmission and post-transmission beliefs to refer to their corresponding densities.
\begin{lemma}\label{lemma:Gupdate}
The estimator's beliefs evolve according to the following fixed transformations:
 \begin{enumerate}
\item $ \Pi_{t+1}(\VEC x,e)  $
\begin{align}
=\lambda^{-n}\int_{\VEC x' \in \mathbb{R}^n}\sum_{e' \in \mathcal{E}} [\mathds{P}(E_{t+1} =e|E'_t = e')\mu(\VEC x - \VEC x')  \Theta_t(\lambda^{-1}\VEC{A}^{-1}\VEC x',e')],
\end{align}
where $\mu$ is the probability density function of $\VEC Z_t$.
~\medskip \\
 We denote this transformation by 
$\Pi_{t+1} = Q^1_{t+1}(\Theta_t)$.
\item 
\begin{align}
\Theta_t(\VEC x,e) =  \left \{ \begin{array}{ll}
               \delta_{\{\VEC x',e'-1\}}~~~ ~~~~~~~~~~~~ \mbox{if $Y_t =(\VEC x',e')$} \\
                ~~  ~~ \\
               \frac{(1-\Gamma_t(\VEC \VEC x,e))\Pi_t(\VEC x,e)}{\int_{\VEC x'}\sum_{e'}(1-\Gamma_t(\VEC x',e'))\Pi_t(\VEC x',e')}  \mbox{ if $Y_t=\epsilon$ }
               \end{array},
               \right.
\end{align} 
where $\delta_{\{x',e'-1\}}$ is a degenerate distribution  at $(x',e'-1)$.
 We denote this transformation by  $\Theta_t = Q^2_t(\Pi_t,\Gamma_t,Y_t)$. 
\end{enumerate}
\end{lemma}
Further, we can establish the following analogue of Theorem \ref{thm:val_functions}
\begin{theorem}\label{thm:mval_functions}
Let $\pi, \theta$ be any pre-transmission and post-transmission belief. Define recursively the following functions:
\begin{equation*}
W_{T+1}(\pi) := 0
\end{equation*}
\begin{align}\label{eq:mdpeq1}
&V_t(\theta) := \inf_{\VEC{a} \in \mathbb{R}^n} \mathds{E}[\norm{\VEC{X}_t - \VEC{a}}^2 + W_{t+1}(\Pi_{t+1})|\Theta_t=\theta] 
\end{align}
 where $\Pi_{t+1} = Q^1_{t+1}(\Theta_t)$ (see Lemma \ref{lemma:Gupdate}), and 
\begin{align} \label{eq:mdpeq2}
&W_{t}(\pi) := \inf_{\tilde\gamma \in \mathcal{G}} \mathds{E}[c\ind_{\{U_t=1\}}+V_{t}(\Theta_{t})|\Pi_t=\pi,\Gamma_t = \tilde\gamma] 
\end{align}

where $\mathcal{G}$ is the set of all measurable functions $\gamma$ from $\mathbb{R}^n \times \mathcal{E}$ to $\{0,1\}$ such that $\gamma(\VEC{x},0) =0, \forall \VEC{x} \in \mathbb{R}^n$.
\par
Strategies that at each time and  for each pre-transmission and post-transmission select a prescription and estimate that achieves the infimum in \eqref{eq:mdpeq1} and \eqref{eq:mdpeq2} are optimal.
%Estimation and prescription strategies $\VEC g^*, \VEC l^*$ that for each v achieves the infimum in \eqref{eq:mdpeq1} and \eqref{eq:mdpeq2} is an optimal strategy.
 %(It can be shown that  the infimum in the definition of the functions $V_t$ and $W_t$  are achieved.)
\end{theorem}

In order to completely characterize the solution of the dynamic program in Theorem \ref{thm:mval_functions}, we define the following relation on the possible realizations of estimator's beliefs.


%THE RELATION CANNOT BE DEFINED IN TERMS OF MARGINALS..OOPS

\begin{definition} [Binary Relation $\RELATION^n$]
Let $\theta$ and $\tilde\theta$ be two post-transmission beliefs.
We say $\theta\RELATION\tilde\theta$ iff:
\begin{enumerate}
%\item[(i)] For each $e \in \mathcal{E}$, $\theta(\cdot,e)$ and $\tilde\theta(\cdot,e)$ are unnormalized pdfs with 
%\[ \int_{\VEC{x}}\theta(\VEC x,e)d \VEC x = \int_{\VEC{x}}\tilde\theta(\VEC x,e)d \VEC x \] 
\item [(i)] For each $e \in \mathcal{E}$, 
$\theta(\cdot,e) \prec \tilde\theta(\cdot,e)$.
\item [(ii)] For all $e \in \mathcal{E}$, $\tilde\theta(\cdot,e)$ is symmetric and unimodal about the same point $ x \in \mathcal{X}$. 
\end{enumerate}
Similar relation holds for pre-transmission beliefs.
\end{definition}
\begin{definition}[Property $\RELATION^n$]
 Let $V$ be a function that maps probability measures on $\mathbb{R}^n\times\mathcal{E}$ to the set of real numbers $\mathbb{R}$. We say that $V$ satisfies Property $\RELATION^n$ iff for any two distributions $\theta$ and $\tilde\theta$,
 \[\theta \RELATION^n \tilde\theta \implies V(\theta) \geq V(\tilde\theta)\]
 
\end{definition}

We can now state the analogue of Claim \ref{claim:one}.

\begin{claim} \label{claim:two}
The value functions in Theorem \ref{thm:mval_functions} $W_t$, $t=1,2,\ldots T+1$, and  $V_t, t=1,2,\ldots,T$, satisfy Property $\RELATION^n$.

\end{claim}
\begin{proof}
See Appendix \ref{sec:Gclaimproof}.
\end{proof}

Because of Claim 2, we can follow arguments similar to those in Section \ref{sec:results} to conclude the following: At time $t=1$, because $\pi_1(\cdot,e)$ is symmetric unimodal about $\VEC 0$ for all $e$, it is sufficient to consider symmetric threshold based prescriptions of the form 
\begin{align}
\gamma(\VEC x,e) = \left \{ \begin{array}{ll}
               1 & \mbox{if $\norm{\VEC x} \geq r_t(e,\pi_1)$} \\
               0 & \mbox{ if $\norm{\VEC x} < r_t(e,\pi_1)$}                
                \end{array}
               \right.
%                   
\end{align} 
in right hand side of equation \eqref{eq:mdpeq1} for time $t=1$. Using such prescriptions implies that $\theta_1(\cdot,e)$ is always symmetric unimodal about some point $\VEC a$ which is the optimal estimate in \eqref{eq:mdpeq2} at time $t=1$. Further, $\pi_2(\cdot,e)$ will also be symmetric unimodal about $\lambda \VEC A \VEC a$ and therefore it is sufficient to restrict to symmetric treshold based prescriptions in \eqref{eq:mdpeq2} at time $t=2$. Proceeding sequentially allows us to rewrite the dynamic program of Theorem \ref{thm:mval_functions} as follows:

\begin{theorem}\label{thm:mval_functions}
Let $\pi, \theta$ be any pre-transmission and post-transmission belief such that $\pi(\cdot,e)$ is symmetric unimodal about $\VEC a(\pi)$ and $\theta(\cdot,e)$ is symmetric unimodal about $\VEC a(\theta)$. Define recursively the following functions:
\begin{equation*}
W_{T+1}(\pi) := 0
\end{equation*}
\begin{align}\label{eq:mdpeq1}
&V_t(\theta) :=  \mathds{E}[\norm{\VEC{X}_t - \VEC a(\theta)}^2 + W_{t+1}(\Pi_{t+1})|\Theta_t=\theta] 
\end{align}
 where $\Pi_{t+1} = Q^1_{t+1}(\Theta_t)$ (see Lemma \ref{lemma:Gupdate}), and 
\begin{align} \label{eq:mdpeq2}
&W_{t}(\pi) := \inf_{\tilde\gamma \in \mathcal{SG}} \mathds{E}[c\ind_{\{U_t=1\}}+V_{t}(\Theta_{t})|\Pi_t=\pi,\Gamma_t = \tilde\gamma] 
\end{align}

where $\mathcal{SG} \subset \mathcal{G}$ is the set of symmetric threshold based prescriptions of the form 
\begin{align}
\gamma(\VEC x,e) = \left \{ \begin{array}{ll}
               1 & \mbox{if $\norm{\VEC x- \lambda \VEC{A}\VEC a(\pi)} \geq r_t(e,\pi)$} \\
               0 & \mbox{ if $\norm{\VEC x- \lambda \VEC{A}\VEC a(\pi)} < r_t(e,\pi)$}                
                \end{array}
               \right.
%                   
\end{align} 
\par
Strategies that at each time and  for each pre-transmission and post-transmission select a prescription and estimate that achieves the infimum in \eqref{eq:mdpeq1} and \eqref{eq:mdpeq2} are optimal.
%Estimation and prescription strategies $\VEC g^*, \VEC l^*$ that for each v achieves the infimum in \eqref{eq:mdpeq1} and \eqref{eq:mdpeq2} is an optimal strategy.
 %(It can be shown that  the infimum in the definition of the functions $V_t$ and $W_t$  are achieved.)
\end{theorem}
 

\begin{theorem}\label{thm:Gmain}
 In Problem \ref{prob:multi_d}, it is without loss of optimality to restrict to  strategies  $\VEC f^*, \VEC g^*$  that are given as:
\begin{align}
g^*_1(y_1) = \left \{ \begin{array}{ll}
               \VEC 0 & \mbox{if $y_1 =\epsilon$} \\
               \VEC x & \mbox{ if $y_1=(\VEC x,e)$ }
               \end{array}
               \right.
\end{align} 
and 
\begin{align}
g^*_t(y_{1:t}) = \left \{ \begin{array}{ll}
                \lambda \VEC{A}\VEC{a} & \mbox{if $y_t =\epsilon$} \\
               \VEC x & \mbox{ if $y_t=(\VEC x,e)$ }
               \end{array}
               \right.
\end{align} 
where $\VEC{a} =g^*_{t-1}(y_{1:t-1})$, and 
\begin{align}
f^*_t(\VEC x,e,y_{1:t-1}) = \left \{ \begin{array}{ll}
               1 & \mbox{if $\norm{\VEC x- \lambda \VEC{A}\VEC a} \geq r_t(e,\pi_t)$} \\
               0 & \mbox{ if $\norm{\VEC x- \lambda \VEC{A}\VEC a} < r_t(e,\pi_t)$}                
                \end{array}
               \right.
%                   
\end{align} 
where $\VEC a = g^*_{t-1}(y_{1:t-1})$, $\pi_t = \mathds{P}(X_t,E_t|y_{1:t-1})$, and $r_t(e,\pi_t) \geq 0$ are thresholds that depend on 

\end{theorem}
Further, the optimal values of thresholds can be obtained by a dynamic program similar to lemma \ref{lemma:sdp}.
\begin{lemma}\label{lemma:Gsdp}
Given that the strategy for the estimator is fixed to $\VEC g^*$,  the best sensor strategy (from the class of all possible strategies) is  of the form 
\[ U_t = f^*_t(\VEC D_t,E_t), \]
where $\VEC D_t := \VEC X_t-g^*_{t-1}(Y_{1:t-1})$. Further, this strategy is described by the following dynamic program:
\begin{equation*}
J_{T+1}(\cdot,\cdot) := 0
\end{equation*}
For positive energy levels $e > 0$,
\begin{align}\label{eq:sdpeq1}
&J_t(\VEC d,e) := \min\{c+\mathds{E}[J_{t+1}(\VEC Z_t,\min(e-1+N_t,B))], \notag \\ &\norm{\VEC d}^2+ \mathds{E}[J_{t+1}(\VEC d+\VEC Z_t,\min(e+N_t,B))] \},
\end{align}
For $e>0$, the optimal action for a realization $(\VEC d,e)$ of $(\VEC D_t,E_t)$ is $U_t=1$ iff $J_t(\VEC d,e)$ is equal to the first term in the right hand side of \eqref{eq:sdpeq1}.
If $e=0$, $J_t(\cdot,0) $ is the second term in the right hand side of \eqref{eq:sdpeq1} evaluated at $e=0$  and the optimal action is $U_t=0$.
\end{lemma} 


\section{Special Cases}
%The model of Sections \ref{sec:PF} and \ref{sec:multi_d} assumed controlled Markovian dynamics of the energy level. 
By making suitable assumptions on the source, the energy storage limit $B$ of the sensor and statistics of initial energy level and the energy harvested at each time, we can derive the following special cases of Problem \ref{prob:main} in Section \ref{sec:PF} and Problem \ref{prob:multi_d} in Section \ref{sec:multi_d}.
\subsubsection{Fixed number of Transmissions}  Assume that the initial energy level $E_1 = K$ ($K \leq B$) with probability $1$ and that the energy harvested at any time $N_t =0$ with probability $1$. Under these assumptions, Problem \ref{prob:main} can be interpreted as the case when the sensor can afford at most $K$ transmissions during the time-horizon with no possibility of energy harvesting. This is similar to the model in \cite{ImerBasar1}.


\subsubsection{No Energy Constraint} Assume that the storage limit $B=1$ and that initial energy level and the energy harvested at each time is $1$ with probability $1$. Then, it follows that at any time $t$, $E_t=1$ with probability $1$. Thus, the sensor is \emph{always guaranteed to have energy to communicate}. Under these assumptions, Problem \ref{prob:main} can be interpreted as the case when the sensor has no energy constraints (it still has energy costs because of the term $cU_t$ in the objective). This is similar to the model in \cite{Martins:2011}.

\subsubsection{IID Source} The analysis of Sections \ref{sec:results} and \ref{sec:multi_d} can be repeated if the source evolution is assumed to be $X_{t+1} = Z_t$, where $Z_t$ are the iid noise variables in the models of Sections \ref{sec:results} and \ref{sec:multi_d}. For iid sources, the optimal estimate is the mean value of the source in case of no transmission.  Also, the dynamic program of lemma \ref{lemma:sdp} can be used for finite valued iid sources by replacing $D_t$ with $X_t$ and changing \eqref{eq:sdpeq1} to
\begin{align}\label{eq:iiddpeq1}
&J_t(d,e) := \min\{c+\mathds{E}[J_{t+1}(X_{t+1},\min(e-1+N_t,B))], \notag \\ &\tilde{\rho}(d)+ \mathds{E}[J_{t+1}({X}_{t+1},\min(e+N_t,B))] \},
\end{align}
Similar dynamic program can be written for the Gaussian source.


==> multi_d.tex <==
\section{Multi-Dimensional Source} \label{sec:multi_d}

In this section, we consider Problem \ref{prob:main} with a discrete vector source. The sensor observes a discrete-time vector Markov process $\VEC{X}_t =(X^1_t,X^2_t,\ldots,X^n_t)$, $t=1,2,\ldots$. The state space of this source process is  $\mathcal{X}^n$ where $\mathcal{X}$ is a finite interval of the set of integers $\mathbb{Z}$.  The energy dynamics for the sensor as the same as in Problem \ref{prob:main}. 

 At the beginning of the time period $t$, the sensor makes a decision about whether to transmit its current observation vector and its current energy level to the estimator or not. We denote by $U_t \in \{0,1\}$ the sensor's decision at time $t$, where $U_t=0$ means no transmission and $U_t=1$ means a decision to transmit. 
The estimator receives a message $Y_t$ from the sensor where
\begin{align}
Y_t = \left \{ \begin{array}{ll}
               (\VEC{X}_t,E_t) & \mbox{if $U_t =1$} \\
               \epsilon & \mbox{ if $U_t=0$ },
               \end{array}
               \right.
\end{align} 
where $\epsilon$ denotes that no message was transmitted.
The estimator produces an estimate $\VEC{\hat{X}}_t = (\hat{X}^1_t,\ldots, \hat{X}^n_t)$ at time $t$ depending on the sequence of messages it received so far. The system operates for a finite time horizon $T$.


We have the following optimization problem.

\begin{problem}
  \label{prob:multi_d}
  For the model described above, given the statistics of the Markov source and the initial energy level $E_1$, the statistics of amounts of energy harvested at each time, the sensor's energy storage limit $B$ and the time horizon $T$,  find  decision strategies $\VEC f, \VEC g$ for the sensor and the estimator that minimize the following expected cost:
  \begin{equation}\label{eq:mcost}
  J(\VEC f, \VEC g) = \mathds{E} \{\sum_{t=1}^T c U_t + \norm{\VEC{X}_t-\VEC{\hat {X}}_t} \},
  \end{equation}
 where $c \geq 0$ is a communication cost and $\norm{\cdot}$ is the Euclidean norm. 
\end{problem}


\begin{definition}
 A function $\nu: \mathbb{Z}^n \mapsto \mathds{R}$  is said to be \emph{almost symmetric and unimodal (a.s.u.)} about a point $\VEC{a} \in \mathbb{Z}^n$, if $\norm{\VEC{x-a}} < \norm{\VEC{y-a}}$ implies that $\nu(\VEC{x}) \geq \nu(\VEC{y})$. An $a.s.u.$ function is said to be completely symmetric and unimodal (c.s.u.) if $\norm{\VEC{x-a}} = \norm{\VEC{y-a}}$ implies that $\nu(\VEC{x}) = \nu(\VEC{y})$.
\end{definition}

\begin{definition}
For any function $\mu$ from $\mathcal{X}^n$ to $\mathbb{R}$, let    $\mu_{\downarrow} = (\mu_{[1]},\mu_{[2]},\ldots,\mu_{[c]})$ denote the non-increasing rearrangement of $\mu$ with $\mu_{[1]}\geq \mu_{[2]} \geq\ldots \geq \mu_{[c]}$, where $c$ is the cardinality of the finite set $\mathcal{X}^n$. Given two such functions $\mu$ and $\nu$, we say that $\nu$ majorizes $\mu$, denoted by, $\mu \prec \nu$, if the following conditions hold:
\begin{align*}
&\displaystyle\sum_{i=1}^{l} \mu_{[i]} \leq \displaystyle\sum_{i=1}^{l} \nu_{[i]}, \mbox{~~~~~~~~~for $1 \leq l \leq c-1$} \\
&\displaystyle\sum_{i=1}^{c} \mu_{[i]} = \displaystyle\sum_{i=1}^{c} \nu_{[i]}
\end{align*}
\end{definition}

We make the following assumptions:
\begin{enumerate}
 %\item [(A3)] The distortion function $\rho(\VEC{x},\VEC{a})$ is  $\sum_{i=1}^n|x^i-a^i|^k$, for some $k>0$.  \\
\item [(A3)] The source evolution is given as:
 \begin{equation} \label{eq:multievolution}
  \VEC{X}_{t+1} = \VEC{X}_t + \VEC{Z}_t 
 \end{equation}
 where $\VEC{Z}_t, t=1,2,\ldots, T-1$ are i.i.d random vectors with finite support, c.s.u. distribution about $\VEC{0}$ and the distribution of the initial state $X_1$ is also finite support and  a.s.u. about $\VEC{0}$.

\end{enumerate}

Following the arguments of Sections \ref{sec:prelim} and \ref{sec:results}, we can establish that the estimator's beliefs evolve in a manner similar to the one-dimensional evolution given in Lemma \ref{lemma:update}. Further, we can establish the following analogue of Theorem \ref{thm:val_functions}
\begin{theorem}\label{thm:mval_functions}
Let $\pi, \theta$ be any PMF defined on $\mathcal{X}^n \times \mathcal{E}$. Define recursively the following functions:
\begin{equation*}
W_{T+1}(\pi) := 0
\end{equation*}
\begin{align}\label{eq:mdpeq1}
&V_t(\theta) := \min_{\VEC{a} \in \mathcal{X}^n} \mathds{E}[\norm{\VEC{X}_t, \VEC{a}} + W_{t+1}(\Pi_{t+1})|\Theta_t=\theta] 
\end{align}
 and 
\begin{align} \label{eq:mdpeq2}
&W_{t}(\pi) := \min_{\tilde\gamma \in \mathcal{G}} \mathds{E}[c\ind_{\{U_t=1\}}+V_{t}(\Theta_{t})|\Pi_t=\pi,\Gamma_t = \tilde\gamma] 
\end{align}

where $\mathcal{G}$ is the set of all functions $\gamma$ from $\mathcal{X}^n \times \mathcal{E}$ to $[0,1]$ such that $\gamma(\VEC{x},0) =0, \forall \VEC{x} \in \mathcal{X}^n$.
\par 
For each realization  of the post-transmission belief at time $t$, the minimizer in \eqref{eq:mdpeq1} exists and gives the optimal estimate  at time $t$; for each realization of the pre-transmission belief, the minimizer in \eqref{eq:mdpeq2} exists  and gives the optimal prescription at time $t$. %(It can be shown that  the infimum in the definition of the functions $V_t$ and $W_t$  are achieved.)
\end{theorem}

In order to completely characterize the solution of the dynamic program in Theorem \ref{thm:mval_functions}, we define the following relation on the distribution over $\mathcal{X}^n \times \mathcal{E}$.


%THE RELATION CANNOT BE DEFINED IN TERMS OF MARGINALS..OOPS

\begin{definition} [Binary Relation $\RELATION^n$]
Let $\theta$ and $\tilde\theta$ be two distributions on $\mathcal{X}^n\times \mathcal{E}$. 
We say $\theta\RELATION\tilde\theta$ iff:
\begin{enumerate}
%\item[(i)] $m_E\theta = m_E\tilde\theta$
\item [(i)] For each $e \in \mathcal{E}$, 
$\theta(\cdot,e) \prec \tilde\theta(\cdot,e)$.
\item [(ii)] For all $e \in \mathcal{E}$, $\tilde\theta(\cdot,e)$ is a.s.u. about the same point $ x \in \mathcal{X}$. 
\end{enumerate}
\end{definition}
\begin{definition}[Property $\RELATION^n$]
 Let $V$ be a function that maps distributions on $\mathcal{X}^n\times\mathcal{E}$ to the set of real numbers $\mathbb{R}$. We say that $V$ satisfies Property $\RELATION^n$ iff for any two distributions $\theta$ and $\tilde\theta$,
 \[\theta \RELATION^n \tilde\theta \implies V(\theta) \geq V(\tilde\theta)\]
 
\end{definition}

We can now state the analogue of Claim \ref{claim:one}.

\begin{claim} \label{claim:two}
The value functions in Theorem \ref{thm:mval_functions} $W_t$, $t=1,2,\ldots T+1$, and  $V_t, t=1,2,\ldots,T$, satisfy Property $\RELATION^n$.

\end{claim}
\begin{proof}
See Appendix \ref{sec:mclaimproof}.
\end{proof}

